Learning N:M Fine-grained Structured Sparse Neural Networks From Scratch

Sparsity in Deep Neural Networks (DNNs) has been widely studied to compress and accelerate the models on resource-constrained environments. It can be generally categorized into unstructured fine-grained sparsity that zeroes out multiple individual weights distributed across the neural network, and structured coarse-grained sparsity which prunes blocks of sub-networks of a neural network. Fine-grained sparsity can achieve a high compression ratio but is not hardware friendly and hence receives limited speed gains. On the other hand, coarse-grained sparsity cannot concurrently achieve both apparent acceleration on modern GPUs and decent performance. In this paper, we are the first to study training from scratch an N:M fine-grained structured sparse network, which can maintain the advantages of both unstructured fine-grained sparsity and structured coarse-grained sparsity simultaneously on specifically designed GPUs. Specifically, a 2:4 sparse network could achieve 2x speed-up without performance drop on Nvidia A100 GPUs. Furthermore, we propose a novel and effective ingredient, sparse-refined straight-through estimator (SR-STE), to alleviate the negative influence of the approximated gradients computed by vanilla STE during optimization. We also define a metric, Sparse Architecture Divergence (SAD), to measure the sparse network's topology change during the training process. Finally, We justify SR-STE's advantages with SAD and demonstrate the effectiveness of SR-STE by performing comprehensive experiments on various tasks. Source codes and models are available at https://github.com/NM-sparsity/NM-sparsity.

==> header.tex <==
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{bm}
\usepackage[textsize=scriptsize]{todonotes}

\newcommand{\gh}[1][j]{\ensuremath{\bm{\hat{g}_{#1}}}}
\newcommand{\mean}[1]{\ensuremath{\mu_{(#1)}}}
\newcommand{\bmean}[1]{\ensuremath{\bm{\mu_{(#1)}}}}
\newcommand{\gs}{\ensuremath{\left(\frac{\gamma}{\sigma_j}\right)}}
\newcommand{\gsm}{\ensuremath{\left(\frac{\gamma}{m\sigma_j}\right)}}
\newcommand{\bmbn}[1][j]{\ensuremath{\bm{\bn}_{#1}}}
\newcommand{\Hess}[1][jj]{\ensuremath{\bm{H}_{{#1}}}}
\newcommand{\z}[1][j]{\ensuremath{z_{#1}}}
\newcommand{\zj}{\ensuremath{z_j}}
\newcommand{\zk}{\ensuremath{z_k}}
\newcommand{\zq}{\ensuremath{z_q}}

\newtheorem*{definition*}{Definition}
\newtheorem*{theorem*}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{fact}[theorem]{Fact}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\corr}{\text{corr}}
\newcommand{\wrt}{w.r.t.\ }

\newcommand{\vz}{\ensuremath{z}}
\newcommand{\vx}{\ensuremath{x}}
\newcommand{\vrhat}{\hat{\ensuremath{r}}}
\newcommand{\vzhat}{\hat{\ensuremath{z}}}
\newcommand{\vr}{\ensuremath{r}}
\newcommand{\va}{\overline{\ensuremath{a}}}
\newcommand{\vw}{\ensuremath{w}}
\newcommand{\vmu}{\ensuremath{\mu}}
\newcommand{\what}{\ensuremath{\widehat{w}}}
\newcommand{\matI}{\ensuremath{I}}
\newcommand{\thetastar}{\ensuremath{\theta^\star}}
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
\newcommand{\normal}{\ensuremath{\mathcal{N}}}
\newcommand{\M}{\ensuremath{\mathcal{M}}}
\newcommand{\rademacher}{\ensuremath{\mathcal{R}}}
\newcommand{\distP}{\ensuremath{\mathcal{P}}}
\newcommand{\powerset}{\ensuremath{\mathscr{P}}}
\newcommand{\perturbB}{\ensuremath{\mathcal{B}}}
\newcommand{\defeq}{\ensuremath{=}}
\newcommand{\intd}{\ensuremath{\text{d}}}
\newcommand{\mix}{\ensuremath{\text{mix}}}
\newcommand{\eqdef}{\defeq}
\newcommand{\sign}{\ensuremath{\text{sgn}}}
\newcommand{\erfc}{\ensuremath{\text{erfc}}}
\newcommand{\pmset}{\ensuremath{\{\pm 1\}}}
\newcommand{\KL}{\ensuremath{D_{\text{KL}}}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\inlinenote}[1]{\textcolor{blue}{Note: #1}}
\newcommand{\I}{\ensuremath{\mathbb{I}}}

\renewcommand{\L}{\mathcal{L}}
\newcommand{\hL}{\widehat{\mathcal{L}}}
\newcommand{\G}{\frac{\partial \mathcal{L}}{\partial \hat{y}_j^{(b)}}}
\newcommand{\Gt}{\frac{\partial \mathcal{L}}{\partial
\hat{y}_j^{(b)}\hat{y}^{(k)}}}
\newcommand{\inp}{x}
\renewcommand{\l}{y}
\newcommand{\bn}{\hat{y}}
\renewcommand{\d}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\inner}[2]{\left\langle{#1},{#2}\right\rangle}
\newcommand{\norm}[1]{\left|\left|{#1}\right|\right|}
\newcommand{\absval}[1]{\left|{#1}\right|}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\p}{\partial}
\renewcommand{\b}[1]{{#1}^{(b)}}
\newcommand{\kk}[1]{{#1}^{(k)}}
\newcommand{\bl}[1]{{#1}^{(l)}}
\newcommand{\dL}[1]{\d{\hL}{#1}}

\newcommand{\vt}{{\ensuremath{\theta}}}
\newcommand{\vtone}{{\ensuremath{\theta_1}}}
\newcommand{\vttwo}{{\ensuremath{\theta_2}}}
\newcommand{\vtd}{{\ensuremath{\theta + \Delta \theta}}}
\DeclarePairedDelimiter{\parens}{\lparen}{\rparen}
\DeclarePairedDelimiter{\brackets}{[}{]}
\renewcommand{\d}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dd}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}



